Predictive Control Barrier Functions: Bridging model predictive control and control barrier functions

In this paper, we establish a connection between model predictive control (MPC) techniques and Control Barrier Functions (CBFs). Recognizing the similarity between CBFs and Control Lyapunov Functions (CLFs), we propose a MPC formulation that ensures invariance and safety without relying on explicit stability conditions. The value function of our proposed MPC is a CBF, which we refer to as the Predictive Control Barrier Function (PCBF), similar to traditional MPC formulations which encode stability by having value functions as CLFs. Our formulation is simpler than previous PCBF approaches and is based on weaker assumptions while proving a similar theorem that guarantees safety recovery. Notably, our MPC formulation does not require the value function to be strictly decreasing to ensure convergence to a safe invariant set. Numerical examples demonstrate the effectiveness of our approach in guaranteeing safety and constructing non-conservative CBFs.

==> Content/linear_Ex1.tex <==
\section{Examples}
\label{sec: exmaples}
% Examples include 2 parts, one to illustrate the convergence property, the other to illustrate the size of encoded safe set
This section first illustrates the convergence property of the proposed MPC problem using an unstable linear example, where the system recovers initially infeasible states. The second example compares the safe invariant set of CBFs computed with different approaches.
\subsection{Illustrative unstable linear Example}
We consider the same setting as the linear example in \cite{Predictive_CBF}. Consider the unstable linear system
\begin{equation}
    x(k+1) = \begin{bmatrix}
        1.05 & 1 \\
        0 & 1
    \end{bmatrix} x(k) + \begin{bmatrix}
        1 \\
        0.5
    \end{bmatrix}u(k)
\end{equation}
which is subject to state constraints $||x||_\infty \leq 1$ and input constraints $||u||_\infty \leq 1$. A local stabilizing lqr controller has the form $u(x) = K_px(k)$ with $K_p = [-0.5592, -0.9445]$. The terminal invariant set is chosen to be $\mathbb{X}_f = \{x \in \mathbb{R}^n:x^TPx \leq \alpha\}$ with $P = \begin{bmatrix}
    5.6648 & 4.8707\\
    4.8707 & 16.3633
\end{bmatrix}, \alpha = 4$. 
By implementing the 2-stage predictive safety filter approach, following Algorithm 1 in \cite{Predictive_CBF}, the system can recover from initial state constraint violation $x_0 \notin \mathbb{X}$, where the proposed control input is infeasible $u = K_px(k) \notin \mathbb{U}$.

In Fig \ref{fig:level set}, we show the state constraints, the safe set $\mathbb{X}_{MPC}^0 = \{x\in \mathbb{R}^n: V^*(x) = 0 \}$ which is the feasible set of the hard-constrained MPC problem as well as the contour lines of the value function $V^*$. In Fig \ref{fig:PSF trajectory}, we demonstrate the recovery of constraint violations from some infeasible initial states. We include the feasible set of the soft-constrained MPC problem, the safe invariant set $\mathbb{X}_{MPC}^0$ and the closed-loop trajectories, whose initial states are sampled randomly from infeasible regions. As guaranteed by Theorem 1 and 2, all the trajectories converge to the safe invariant set of the hard-constrained MPC problem.
\begin{figure}[ht]
    \centering   \includegraphics[width=0.45\textwidth]{Figure/linear1/correct control invariant set.png}
    \caption{This is a filled contour plot of the value function $V^*$. The level sets of the value function $V^*$ are marked with black dashed lines. The zero level set corresponds to the predictive safe set $\mathbb{X}_{MPC}^0.$ The state space $\mathbb{X}$ is denoted with the red dashed line.}
    \label{fig:level set}
\end{figure}
\begin{figure}[ht]
    \centering   \includegraphics[width=0.4\textwidth]{Figure/linear1/PSF trajectory.png}
    \caption{The feasible set $\mathbb{X}_{MPC}$ of the soft-constrained MPC is marked out by the white external region. Closed-loop trajectories with randomly sampled initial conditions all converge to the safe invariant set within $\mathbb{X}$.}
    \label{fig:PSF trajectory}
\end{figure}

In the following two plots, we compare the  predictive safe set created by our formulation with the one described in \cite{Predictive_CBF} with constraint tightening parameter $\Delta_i = i \cdot 0.05, i \cdot 0.02, i \cdot 0.005$. From Fig \ref{fig:Contour comparison}, it is evident that the contours nearly coincide. When zooming in, we observe that as the tightening parameter decreases, the contours converge to the safe set $\mathbb{X}_{MPC}^0$, which approximates of the maximum invariant set within $\mathbb{X}$.
\begin{figure}[ht]
    \centering   \includegraphics[width=0.4\textwidth]{Figure/contour comparison.png}
    \caption{Compare the variations in the safe set when applying the formulation from \cite{Predictive_CBF} with different constraint tightening parameters: $\Delta_i = i \cdot 0.05$ (blue dashed line), $i \cdot 0.02$ (blue solid line), $i \cdot 0.005$ (blue dotted line), versus our formulation without constraint tightening (green solid line). }
    \label{fig:Contour comparison}
\end{figure}
\begin{figure}[ht]
    \centering   \includegraphics[width=0.4\textwidth]{Figure/contour comparison detail.png}
    \caption{Zoom in to see the difference in the safe set. When the tightening parameter decreases, the zero level set extend and eventually converge to that of our formulation.}
    \label{fig:Detailed contour comparison}
\end{figure}



==> Content/new.tex <==
\begin{abstract}
In this paper, we connect model predictive control (MPC) techniques and Control Barrier Functions (CBFs). By noticing the similarity between CBFs and Control Lyapunov Functions (CLFs), we propose a safe MPC method that ensures invariance and safety independent of any stability objectives. The value function of the safe MPC is a CBF, termed as Predictive Control Barrier Function (PCBF). Unlike the previous PCBF formulations, our formulation is simpler and uses milder assumption to prove analogous theorem that guarantees safety recovery. Specifically, our safe MPC formulation does not require a strictly decreasing value function to guarantee convergence to the safe invariant set. Numerical examples illustrate the recovery process and demonstrate the effectiveness of our formulation in constructing non-conservative CBFs.
\end{abstract}



%% Old abstract
\begin{abstract}
We propose a Model Predictive Control (MPC) method that ensures invariance and safety independent of any stability objectives. Implementing non-conservative safe controllers, using techniques based on control barrier functions is challenging.
%
% \PGnote{I don't understand what this means.   \emph{Defining} non-conservative safety constraints seems easy.   It is respecting them that is difficult.    Maybe we want something like ``implementing non-conservative controllers, using techniques based on control barrier functions, that respect safety constraints is challenging''?}
%
%
It is useful not only to identify the safe invariant set but also to act as a recovery procedure to guide trajectories to converge to it, especially given that the safe invariant set can sometimes be overly restrictive. To address this, our formulation extends the safe invariant set beyond a predefined conservative safe set and guarantees convergence from initially unsafe regions to the maximal safe invariant set. This approach effectively bridges the gap between CBFs and MPC, where the proposed MPC implicitly encodes a CBF, similar to how MPC for stability implicitly encodes a Control Lyapunov Function (CLF). Numerical examples illustrate the recovery process and demonstrate the effectiveness of our formulation in constructing non-conservative CBFs.
\end{abstract}

==> Content/redundant_info.tex <==
\begin{abstract}
We propose a Model Predictive Control (MPC) method that ensures invariance and safety independent of any stability objectives. Implementing non-conservative safe controllers, using techniques based on control barrier functions is challenging.
%
% \PGnote{I don't understand what this means.   \emph{Defining} non-conservative safety constraints seems easy.   It is respecting them that is difficult.    Maybe we want something like ``implementing non-conservative controllers, using techniques based on control barrier functions, that respect safety constraints is challenging''?}
%
%
It is useful not only to identify the safe invariant set but also to act as a recovery procedure to guide trajectories to converge to it, especially given that the safe invariant set can sometimes be overly restrictive. To address this, our formulation extends the safe invariant set beyond a predefined conservative safe set and guarantees convergence from initially unsafe regions to the maximal safe invariant set. This approach effectively bridges the gap between CBFs and MPC, where the proposed MPC implicitly encodes a CBF, similar to how MPC for stability implicitly encodes a Control Lyapunov Function (CLF). Numerical examples illustrate the recovery process and demonstrate the effectiveness of our formulation in constructing non-conservative CBFs.
\end{abstract}

\section{Abstract}
We validate our approach through simulations, comparing the invariant safe set of our MPC-based CBFs with other methods such as backup CBF, sum-of-squares (SOS), and Hamilton-Jacobi (HJ) reachability approaches. Additionally, we demonstrate the convergence properties and show how they can be integrated within a predictive safety filter using a 2-stage algorithm.

\section{Introduction}
% comment out from the introduction section
While learning-based control performs exceptionally at complex tasks, ensuring safety remains unsolved. Safe reinforcement learning aims to balance performance and safety \cite{Safe_RL},  struggling to provide provable safety guarantees.

Safety filters offer a modular framework to provide safety guarantees independent of any pre-selected controller \cite{Safety_filter_overview}.

There are three common methods used to construct the safety filter: reachability-based methods \cite{Recent_reachability}, \cite{Reachability_overview}, control barrier functions (CBFs) \cite{Alan2022ControlBF}, \cite{CBF_theory_and_application}, and predictive control techniques \cite{PSF_origin, PSF_paper, Predictive_CBF, Safety_filter_overview}. These methods are all based on set invariance, ensuring a system remains within a specific set throughout its evolution. 


The motivation behind our work is to develop an MPC formulation that guarantees invariance, with its value function serving as a control barrier function, similar to how MPC is used to ensure stability with its value function acting as a Lyapunov function. This idea stems from recognizing the similarities between the definitions of Control Barrier Functions and Control Lyapunov Functions. 

Unlike \cite{Predictive_CBF}, which enlarges the feasible region with a softened auxiliary predictive control problem and uses state constraint tightening for recovery from an unsafe state, our formulation does not require tightening.The soft-constrained MPC problem uses penalty functions to lift state constraints into objective functions and the resulting value function is a ZCBF.  In contrast, using barrier functions to lift state constraints would yield a reciprocal control barrier function (RCBF). 

MPC will be used to expand the domain of CBFs to include points in unsafe regions that will eventually converge to the safe invariant set. In this process, the resulting value function of the underlying optimal control problem is also a CBF with an enlarged domain, and all trajectories that start within the domain will converge to the safe invariant set.

In \cite{backup_CBF}, it introduces backup CBF which propagates a nominal trajectory on a receding horizon and uses a predetermined backup control policy $\pi$ to enlarge the known control invariant set. However, the size of the enlarged invariant set depends on the choice of backup policy. We provide an example to compare the invariant safe set of MPC-based CBF with other methods, such as backup CBF, SOS \cite{SOS_formulation}, Multi-Parametric Programming \cite{MPT3}, and HJ PDE \cite{HJ_formulation}. 

To address this, an alternative approach is to identify a (potentially conservative) candidate invariant set characterizable by a control barrier function (CBF) \cite{Alan2022ControlBF, CBF_theory_and_application}. CBFs are functions that are negative in the unsafe set, with their zero-level set representing the safe invariant set and can be constructed through a variety of methods including sum-of-squares techniques \cite{SOS_formulation} and learning-based-certificates \cite{robey2020learningcontrolbarrierfunctions}. However, these methods usually yield overly conservative CBFs, and efficient construction of guaranteed and non-conservative CBFs remains an open challenge.

Unlike traditional MPC convergence proofs that rely on Lyapunov's theorem, we apply the invariant set theorem for continuous-time system described in section 3.4 of \cite{Nonlinear_Control_Book} to our discrete-time system. The invariant set theorem requires weaker conditions than Lyapunov's theorem while achieving analogous outcomes. 
\PGnote{It's not clear what the `invariant set theorem' being referred to is, and the citation is to a book.  Provide a more specific reference and description here.

Also, `same outcome' as what?   The outcome is not a stability proof.   Maybe you mean something like `analagous outcome' or `similar result'?
}

Using Lyapunov’s theorem necessitates state constraint tightening along the prediction horizon to guarantee a strictly decreasing value function and therefore prove for convergence \cite{Predictive_CBF}. 
\PGnote{Do you mean `tightening' here, or do you mean that constraints just can't be softened?}


In our approach, the MPC value function serves as a CBF, with its zero-level set representing the invariant set. The formulation extends a small, conservative control invariant set into a much larger one by solving a receding-horizon open-loop control problem. 

% No need to include too much information about the numerical simulation in the introduction
Our numerical examples demonstrate that the control invariant sets derived from the value functions, termed as the predictive control barrier functions (PCBF), closely approximate the maximal control invariant set. 
% \PGnote{Final sentence doesn't really belong here.   Maybe some direct statement like this is good to make, but probably in the abstract or very early in the introduction.}

Our soft-constrained MPC problem can also be used as an auxiliary problem \cite{Predictive_CBF} alongside a predictive safety filter (PSF) \cite{PSF_origin, PSF_paper,  Safety_filter_overview}, enabling constraints recovery, as we illustrate in Section~\ref{sec: exmaples}. 



\section{Preliminary}
\textbf{Definition II.3 (Forward Invariance).} \cite{ZCBF} A set $C \subset \mathbb{R}^n$ is forward invariant if for every $x(0) \in C$, the solution $x(k)$ of \eqref{closed_loop_system} satisfies $x(k) \in C$ for all $k \geq 0$.

\section{Safe MPC}
To ensure recursive feasibility of the above MPC formulation, we impose the following assumptions \cite{MPC_optimality}, which are commonly used in MPC analysis.
\newline
\textbf{Assumption 1:} State constraints are satisfied in the terminal set, i.e., $\mathbb{X}_f \subset \mathbb{X}$ and $\mathbb{X}_f$ is compact. 
\newline
\textbf{Assumption 2:} Input constraints are satisfied in $\mathbb{X}_f$, i.e., there exists a local controller $\kappa_f: \mathbb{X}_f \rightarrow \mathbb{U}, \; \forall x \in \mathbb{X}_f$.
\newline
\textbf{Assumption 3:} $\mathbb{X}_f$ is positively invariant under $\kappa_f(\cdot)$, i.e., $f(x, \kappa_f(x)) \in \mathbb{X}_f, \forall x \in \mathbb{X}_f$.
% \newline The assumption below has moved to section 2
% \textbf{Assumption 4:} $\mathbb{X}$ is a polyhedron in $\mathbb{R}^n$. $\mathbb{U}$ is a polytope in $\mathbb{R}^m$, hence is compact and convex.
\newline
\textbf{Assumption 4:} Both the soft-constrained and hard-constrained MPC problem are feasible, i.e., $\mathbb{X}^{\xi}_{MPC},  \mathbb{X}_{MPC}^0$ are non-empty.% and compact sets.
